A Retrospective Analysis of User Exposure to (Illicit) Cryptocurrency Mining on the Web

In late 2017, a sudden proliferation of malicious JavaScript was reported on the Web: browser-based mining exploited the CPU time of website visitors to mine the cryptocurrency Monero. Several studies measured the deployment of such code and developed defenses. However, previous work did not establish how many users were really exposed to the identified mining sites and whether there was a real risk given common user browsing behavior. In this paper, we present a retroactive analysis to close this research gap. We pool large-scale, longitudinal data from several vantage points, gathered during the prime time of illicit cryptomining, to measure the impact on web users. We leverage data from passive traffic monitoring of university networks and a large European ISP, with suspected mining sites identified in previous active scans. We corroborate our results with data from a browser extension with a large user base that tracks site visits. We also monitor open HTTP proxies and the Tor network for malicious injection of code. We find that the risk for most Web users was always very low, much lower than what deployment scans suggested. Any exposure period was also very brief. However, we also identify a previously unknown and exploited attack vector on mobile devices.

==> tikzlibrarytimeline.code.tex <==
% * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *
% COPYRIGHT 2014 - Claudio Fiandrino
% Released under the LaTeX Project Public License v1.3c or later
% 
% email: <claudio dot fiandrino at gmail dot com>
%
% Timeline TikZ library version 0.3a - 19/07/2014

\usetikzlibrary{backgrounds,calc}

\pgfkeys{/tikz/.cd,
  timespan/.store in=\timespan,
  timespan=,
  timeline width/.store in=\timelinewidth,
  timeline width=20,
  timeline height/.store in=\timelineheight,
  timeline height=1,
  timeline offset/.store in=\timelineoffset,
  timeline offset=0.15,
  initial week/.store in=\initialweek,
  initial week=1,
  end week/.store in=\endweek,
  end week=2,
  time point/.store in=\timepoint,
  time point=0.5,
  between day/.style args={#1 and #2 in #3}{% auxiliary style for days
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between week/.style args={#1 and #2 in #3}{% style for weeks
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between month/.style args={#1 and #2 in #3}{% auxiliary style for months
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between year/.style args={#1 and #2 in #3}{% auxiliary style for years
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  involvement degree/.store in=\involvdegree,
  involvement degree=2cm,
  phase color/.store in=\phasecol,
  phase color=red!50!orange,
  phase appearance/.style={
    circle,
    opacity=0.3,
    minimum size=\involvdegree,
    fill=\phasecol
  },
}
% settings to customize aspect of timeline
\newif\ifcustominterval
\pgfkeys{/tikz/timeline/.cd,
  custom interval/.is if=custominterval,
  custom interval=false,
}

% settings to deploy milestones
\pgfkeys{/tikz/milestone/.cd,
  at/.store in=\msstartpoint,
  at=phase-1.north,
  circle radius/.store in=\milestonecircleradius,
  circle radius=0.1cm,
  direction/.store in=\msdirection,
  direction=90:2cm,
  text/.store in=\mstext,
  text={},
  text options/.code={\tikzset{#1}},
}

\newcommand{\reftimespan}{\MakeLowerCase{\timespan}}


% Change this to change the black bar behind the timeline
\newcommand{\timeline}[2][]{
  \pgfkeys{/tikz/timeline/.cd,#1}
  %\draw[fill,opacity=0.4] (0,0.3\timelineheight) rectangle (\timelinewidth,0.7\timelineheight);
  \draw[fill,opacity=1] (0,0.55) rectangle (\timelinewidth,0.6);
% Shaders (fade effects in the bar)
 % \shade[opacity=0,top color=black, bottom color=white,middle color=white!20]
 %   (0,0) rectangle (\timelinewidth,-\timelineoffset);
 % \shade[opacity=0,top color=white, bottom color=white,middle color=white!20]  
 %   (0,\timelineheight) rectangle (\timelinewidth,\timelineheight+\timelineoffset);

  \ifcustominterval%
    \foreach \smitem [count=\xi] in {#2}  {\global\let\maxsmitem\xi}%
  \else%
    \foreach \smitem [count=\xi] in {1,...,#2}  {\global\let\maxsmitem\xi}%
  \fi%
  
  \pgfmathsetmacro\position{\timelinewidth/(\maxsmitem+1)}
  \node at (0,0.5\timelineheight)(\timespan-0){\phantom{Week 0}};
 
  \ifcustominterval%
    \foreach \x[count=\xi] in {#2}{%
      %\node[text=white,text depth=0pt]at +(\xi*\position,0.5\timelineheight) (\timespan-\xi) {\timespan\ \x};%
      \node[text=black,text depth=0pt]at +(\xi*\position,0.9\timelineheight) (\timespan-\xi) {\timespan\ \x};%
      \path[-, thick] (\xi*\position, 0.7) edge (\xi*\position, 0.45);
    }%
  \else%
    \foreach \x[count=\xi] in {1,...,#2}{%
      %\node[text=white, text depth=0pt]at +(\xi*\position,0.5\timelineheight) (\timespan-\xi) {\timespan\ \x};%
      \node[text=black, text depth=0pt]at +(\xi*\position,0.5\timelineheight) (\timespan-\xi) {\timespan\ \x};%
      \path[-, thick] (\xi*\position, 0.3) edge (\xi*\position, 0.1);
    }%
  \fi%  
}

\newcounter{involv}
\setcounter{involv}{0}

\newcommand{\phase}[1]{
\stepcounter{involv}
\node[phase appearance,#1] 
 (phase-\theinvolv)
 at ($(\timespan-\initialweek)!\timepoint!(\timespan-\endweek)$){};
}

\newcommand{\initialphase}[1]{
\node[phase appearance,#1,anchor=west,between week=0 and 1 in 0,] 
 (phase-\theinvolv)
 at ($(\timespan-0)!0!(\timespan-1)$){};
\setcounter{involv}{0} 
}

\newenvironment{phases}{\begin{pgfonlayer}{background}}{\end{pgfonlayer}}

\newcommand{\addmilestone}[1]{
\pgfkeys{/tikz/milestone/.cd,#1}
\draw[double,fill] (\msstartpoint) circle [radius=\milestonecircleradius];
\draw(\msstartpoint)--++(\msdirection)node[/tikz/milestone/text options]{\mstext};
}

% HISTORY
% 0.1 -> initial release
% 0.2 -> customizable timespan label
% 0.3 -> \timeline command with custom intervals
%             styles ``between x''
%             removed unnecessary call to xstring
% 0.3a -> text depth for timeline labels

